Discrete Optimization for Unsupervised Sentence Summarization with Word-Level Extraction

Automatic sentence summarization produces a shorter version of a sentence, while preserving its most important information. A good summary is characterized by language fluency and high information overlap with the source sentence. We model these two aspects in an unsupervised objective function, consisting of language modeling and semantic similarity metrics. We search for a high-scoring summary by discrete optimization. Our proposed method achieves a new state-of-the art for unsupervised sentence summarization according to ROUGE scores. Additionally, we demonstrate that the commonly reported ROUGE F1 metric is sensitive to summary length. Since this is unwillingly exploited in recent work, we emphasize that future evaluation should explicitly group summarization systems by output length brackets.

==> tables/data_stats.tex <==
\begin{table}[]
\centering
\begin{tabular}{l|r|r|r}
\hline
Gigaword & \multicolumn{1}{c|}{\textbf{\#}} & \multicolumn{1}{c|}{\textbf{$\varnothing$source}} & \multicolumn{1}{c}{\textbf{$\varnothing$target}} \\ \hline
train    & 3.8M                        & 31.3                                               & 8.2                                                \\
test     & 1951                             & 29.6                                               & 8.7                                                \\ \hline
DUC2004  & 500                              & 35.5                                               & 10.4                                               \\ \hline
\end{tabular}
\caption{Statistics of Gigaword dataset for headline generation \citep{rush2015neural} and DUC2004 data \citep{over2004introduction}. \textit{\#}: number of instances. \textit{$\varnothing$source}: average number of words in the source sentence. \textit{$\varnothing$target}: average number of words in the target summary.}
\label{table:data_stats}
\end{table}
